Interoperability of statistical models in pandemic preparedness: principles and reality

We present "interoperability" as a guiding framework for statistical modelling to assist policy makers asking multiple questions using diverse datasets in the face of an evolving pandemic response. Interoperability provides an important set of principles for future pandemic preparedness, through the joint design and deployment of adaptable systems of statistical models for disease surveillance using probabilistic reasoning. We illustrate this through case studies for inferring spatial-temporal coronavirus disease 2019 (COVID-19) prevalence and reproduction numbers in England.

==> graphs/debias_import_across_weeks_regions.tex <==
\begin{figure}[ht]
	\vspace{.4cm}
\begin{center}
    \begin{tikzpicture}
		\def\xlab{2.5cm}
		\def\ylab{1.2cm}
		\node[obs] (debiased) {$p(\nttlocal \mid \mlocal_t)$};
 		\node[latent, left=of debiased] (infs) {$\infs_t^\localsuper$};
 		\node[obs, below=of debiased] (data) {$\data_t^\localsuper$};
 		\node[latent, left=of data, xshift = -.75cm] (theta) {$\datapar_t^\localsuper$};
 		\edge {infs} {debiased}; 
 		\edge[dashed] {infs} {data}; 
 		\edge {theta} {data}; 
%  		\plate {rtplate} {(infs)(data)(debias)} {{$r,t$}}
	\end{tikzpicture}
\end{center}
\vspace{-.25cm}
	\caption{ Interoperable model based on a debiased prevalence likelihood. This DAG is specific to an LTLA $r$, week $t$. The debiased data likelihood $p(\nttlocal \mid \mlocal_t)$ is a probability mass function on prevalence bins. Each bin comprises a range of $\infs$ in population of size $M$. The dashed line represents constraining feedback of information from $\data$ to $\infs$}
	\label{fig:prev_incid_latent}
\end{figure}


==> graphs/simple_debias_import.tex <==
\begin{figure}[ht]
	\vspace{.4cm}
\begin{center}
    \begin{tikzpicture}
		\def\xlab{2.5cm}
		\def\ylab{1.2cm}
		\node[obs] (debiased) {$p(\ntofN \mid \m)$};
 		\node[latent, left=of debiased] (infs) {$\infs$};
 		\node[obs, below=of debiased] (data) {$\data$};
 		\node[latent, left=of data, xshift = -.75cm] (theta) {$\datapar$};
 		\edge {infs} {debiased}; 
 		\edge[dashed] {infs} {data}; 
 		\edge {theta} {data}; 
%  		\plate {rtplate} {(infs)(data)(debias)} {{$r,t$}}
	\end{tikzpicture}
\end{center}
\vspace{-.25cm}
	\caption{Interoperable model based on a debiased prevalence likelihood, implicitly specific to an LTLA $r$, week $t$. The dashed line represents that we wish to constrain feedback of information from $\data$ to $\infs$. Ideally this will be semi-modular inference allowing a full range of partial feedback between the no feedback ``cut'' model, and the full feedback fully Bayesian inferential model (an undashed directed edge). The debiased data likelihood $p(\ntofN \mid \m)$ is a probability mass function on prevalence bins. Each bin comprises a range of $\infs$ in population of size $M$.}
	\label{fig:simple_debias_interoperable}
\end{figure}


==> latex_preamble/goals_tasks_preamble.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Goals and tasks 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{xcolor}
\newcounter{goal}
\setcounter{goal}{0}
\newcounter{task}[goal]
\setcounter{task}{1}
\renewcommand{\thetask}{Task~\,\thegoal.\arabic{task}} 
\newcommand{\goalsection}[1]{\stepcounter{goal} \bigskip \hrule 
                  \section*{Goal \thegoal: #1}}
\newenvironment{task}[1]
   {\refstepcounter{task} \bigskip \noindent {\textbf{\thetask:\  #1.}}}{\par}
\newenvironment{plan}
   {\medskip \noindent \hspace{.5cm} \begin{sf}\textbf{Plan}:\  }
   {\medskip \end{sf}\leavevmode\newline}
\newenvironment{team}
   {\medskip \noindent \hspace{.5cm} \begin{sf}\textbf{Team}:\  }
   {\medskip \end{sf}\leavevmode\newline}
\newenvironment{work}
   {\medskip \noindent \hspace{.5cm} \begin{sf}\textbf{Own it!}:\  }
   {\medskip \end{sf}\leavevmode\newline}


==> latex_preamble/reviewer_response_commands.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Reviewer response commands and environments
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% package needed for optional arguments
\usepackage{xifthen}
% define counters for reviewers and their points
\newcounter{reviewer}
\setcounter{reviewer}{0}
\newcounter{point}[reviewer]
\setcounter{point}{0}

% This refines the format of how the reviewer/point reference will appear.
\renewcommand{\thepoint}{C\,\thereviewer.\arabic{point}} 

% command declarations for reviewer points and our responses
\newcommand{\reviewersection}[1]{\stepcounter{reviewer} \bigskip \hrule
                  \section*{#1}}

\newenvironment{point}
   {\refstepcounter{point} \bigskip \noindent {\textbf{Comment~\thepoint} } ---\ }
   {\par }

\newcommand{\shortpoint}[1]{\refstepcounter{point}  \bigskip \noindent 
	{\textbf{Point~\thepoint} } ---~#1\par }

\newenvironment{reply}
   {\medskip \noindent \begin{sf}\textbf{Impact}:\  }
   {\medskip \end{sf}}

\newcommand{\shortreply}[2][]{\medskip \noindent \begin{sf}\textbf{Reply}:\  #2
	\ifthenelse{\equal{#1}{}}{}{ \hfill \footnotesize (#1)}%
	\medskip \end{sf}}


==> latex_preamble/text_referencing_commands.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Text referencing commands
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\R}[1]{\label{#1}\linelabel{#1}}
\newcommand{\lrg}[1]{page \pageref{#1} line \lineref{#1}}
\newcommand{\lr}[2]{page \pageref{#1}, lines~\lineref{#1}-\lineref{#2}}
\newcommand{\lrG}[1]{page \pageref{#1}, lines~\lineref{start_#1}-\lineref{end_#1}}
\newcommand{\reftext}[1]{\begin{quote}\textit{\ref{#1}} \textit{(\lrG{#1})}\end{quote}}
\newcommand{\reflines}[1]{\emph{(\lrG{#1})}}
\renewcommand\tableofcontents{%
	\@starttoc{toc}%
}
\newcommand{\incfigs}{2}
\graphicspath{{../}}
\makeatletter
\def\input@path{{../}}
\makeatother
\makeatletter
\newcommand{\customlabel}[2]{%
	\protected@write \@auxout {}{\string \newlabel {#1}{{#2}{\thepage}{#2}{#1}{}} }%
	\hypertarget{#1}{#2}
}
\makeatother
\renewcommand{\baselinestretch}{\bls} 
\makeatletter
\newcommand*{\newreptext}[1]{%
	\begingroup % babel shorthand support
	\csname @safe@actives@true\endcsname
	\expandafter\endgroup
	\expandafter\newcommand\csname reptext@#1\endcsname
}
\newcommand*{\reptext}[1]{%
	\begingroup
	\csname @safe@actives@true\endcsname % babel shorthand support
	\@ifundefined{reptext@#1}{%
		\@latex@error{\string\reptext{#1} is undefined}\@ehc
		\endgroup
		\textbf{??}%
	}{%
		\endgroup
		\@nameuse{reptext@#1}%
	}%
}
\makeatother
\makeatletter
\newcommand*{\labeltext}[2]{%
	\begingroup
	\def\@currentlabel{#2}%
	\label{#1}%
	\endgroup
	\linelabel{start_#1}
	#2%
	\linelabel{end_#1}
}
\makeatother
\newcommand{\src}[2]{\expandafter\edef\csname #1 \endcsname{#2}}


